Visuomotor Robotic Pruning in Planar Orchards Using Hybrid Reinforcement Learning

Dormant tree pruning is labor-intensive yet essential for maintaining modern high-productivity fruit orchards. In this work, we focus on pruning of modern planar tree training systems - V-Trellis apples and UFO cherries - where trunks and primary branches are trained into approximately planar walls. We introduce an end-to-end pipeline to learn a closed-loop visuomotor controller for robotic pruning. This controller is trained entirely using simulation and synthetically generated data and deployed in real orchards in a zero-shot manner. The pipeline comprises synthetic generation of planar orchard tree meshes, construction of a physics-based orchard simulator, automated collection of successful pruning trajectories via motion planning, and policy learning with a novel hybrid reinforcement-learning algorithm that combines offline demonstrations with online simulated rollouts. The controller uses optical-flow inputs from a wrist-mounted camera - avoiding the need for full 3D-reconstruction - and continuously guides the cutter through cluttered branch environments to a specified cutpoint with correct tool orientation. In exhaustive simulated task-space evaluations over 3,000 pruning points, the policy attains 49.9% success on V-Trellis apples and 46.0% on UFO cherries. We validate the learned controller across 38 physical trials - comprising 28 outdoor field trials in commercial and experimental orchards and 10 indoor laboratory tests - demonstrating zero-shot sim-to-real transfer. The learned policy also outperforms a classical RRT-Connect baseline on physical hardware in laboratory trials.

==> figures/12_analysis_plots.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{images/merged_analysis_plots.png}
    \caption{Failure analysis based on branch orientation. The Azimuth is the branch's orientation with respect to the ground plane; $\pm$ 90 degree is pointing toward/away from the robot. The Elevation axis is the vertical pointing direction, from pointing at the ground (-90 degree) to pointing at the sky (90 degree). \textit{(Top)} V-Trellis. \textit{(Bottom)} UFO. For each tree type left to right. (a) pointing angle error, (b) perpendicular angle error, (c) success rate}
    \label{fig:analysis_plots}
\end{figure*}

==> sections/11_analysis.tex <==
\section{Analysis}
\label{sec:analysis}
\input{figures/12_analysis_plots}
Since the simulation experiments in Section~\ref{sec:experiments:policy}.\ref{sec:experiments:sim} revealed that the dominant sources of error arise from orientation rather than position, we further analyze the visuomotor policy by studying its orientation-dependent error modes. We generate evaluation episodes in simulation with uniform coverage over to-be-pruned branch orientations for both the V-Trellis and UFO architectures. Branch orientation are parametrized in terms of their azimuth and elevation angles, which are discretized into 10-degree bins over each axis for a total of $18\times36$ cells. For each cell, we randomly select three branches whose orientations fall within the corresponding angular ranges and place them at distinct spatial locations in the task space by translating their trees. The results are shown in Figure~\ref{fig:analysis_plots} where elevation is the angle in the vertical plane (90 degree${\rightarrow}$straight up), and azimuth is the rotation in the horizontal plane (90 degree${\rightarrow}$straight at the robot). We report the mean pointing errors (left column), perpendicular errors (middle column) and success rate (right column) for each cell for both V-Trellis (Top row) and UFO (bottom row) architectures. We omit studying the euclidean error here.

In previous work by Jain et al.\cite{JainRL}, a structured error pattern with two prominent regions of large errors centered around $0^\circ$ elevation and $\pm145^\circ$ azimuth were observed. With the addition of an aligned pruner and improved exploration through the inclusion of offline data, these highly structured error modes have disappeared. We now observe more uniform pointing and success errors distributed across all orientation cells.

